Accelerating Deep Learning Inference via Freezing

Over the last few years, Deep Neural Networks (DNNs) have become ubiquitous owing to their high accuracy on real-world tasks. However, this increase in accuracy comes at the cost of computationally expensive models leading to higher prediction latencies. Prior efforts to reduce this latency such as quantization, model distillation, and any-time prediction models typically trade-off accuracy for performance. In this work, we observe that caching intermediate layer outputs can help us avoid running all the layers of a DNN for a sizeable fraction of inference requests. We find that this can potentially reduce the number of effective layers by half for 91.58% of CIFAR-10 requests run on ResNet-18. We present Freeze Inference, a system that introduces approximate caching at each intermediate layer and we discuss techniques to reduce the cache size and improve the cache hit rate. Finally, we discuss some of the open research challenges in realizing such a design.

==> conclusion.tex <==
In this paper we introduced Freeze Inference, a general technique to improve the latency of serving deep learning models. By building an approximate cache for each intermediate layer, we show that we can avoid running all the layers of a DNN for a large fraction of requests. We present results from our initial prototype and outline some of the research challenges in realizing such a design.  

==> optimizations.tex <==
\label{sec:optimizations}

Freeze Inference can overcome the computational and memory overheads by leveraging the fact that intermediate layer points are semantically related to each other (Figure \ref{fig:clustering}). In this light, we can use $k$-means to cluster neighboring intermediate layer points and represent them by a single cluster center. This reduces the number of points that need to be stored in the cache and consequently reduces both the computational complexity and memory overheads.

To enable this change, we need to augment the cache structure. We construct a per-layer cache such that each item consists of a cluster center, the majority label in that cluster, and the fraction of majority label. During inference, the output of an intermediate layer first undergoes dimensionality reduction and is then queried against the cache. The cache look-up iterates through the set of cluster centers and finds the closest cluster center. The API returns the majority label of that cluster as the predicted label and the ratio of the fraction of majority label to distance from the cluster center as the confidence value.

\begin{figure}
\centering
    \subfloat[ResNet-18 ($k$=100)]{\includegraphics[width=0.49\columnwidth]{kmeans_resnet18.png}} \label{fig:upper_bound}
    \subfloat[ResNet-50 ($k$=1000)]{\includegraphics[width=0.49\columnwidth]{kmeans_resnet50.png}} \label{fig:knn_res18}
\caption{\label{fig:kmeans}
\footnotesize
CDF of blocks at which predictions are frozen using $k$-means
}
\end{figure}
Figure \ref{fig:kmeans} shows the distribution of layers at which inference requests are $frozen$ using the $k$-means clustering approach for ResNet-18 and ResNet-50. For ResNet 18, we observe that with k-means Freeze Inference saves half the computation for about 60\% and 25\% of the points on CIFAR-10 and CIFAR-100 respectively. Similarly, for ResNet-50, we are able to save half the computation for 46.26\% and 25.81\% of the points on CIFAR-10 and CIFAR-100 respectively. Overall, this approach achieves an accuracy of 92.85\% and 88.86\% with respect to the model's prediction for CIFAR-10 and CIFAR-100 datasets respectively. Our experiments show that cache look-up is about 20$X$ faster than the compute for a single layer. Additionally, from Table \ref{tab:memory_reqs} we see that the cache requires a mere 12.5MB of memory for ResNet-18. Thus, $k$-means solves the problems both with respect to computational complexity and memory requirements.


==> todo.tex <==

\begin{itemize}
  \item Cite compression work : https://arxiv.org/pdf/1510.00149v5.pdf
  \item 
\end{itemize}
